Brain-inspired Cognition in Next Generation Racetrack Memories

Hyperdimensional computing (HDC) is an emerging computational framework inspired by the brain that operates on vectors with thousands of dimensions to emulate cognition. Unlike conventional computational frameworks that operate on numbers, HDC, like the brain, uses high dimensional random vectors and is capable of one-shot learning. HDC is based on a well-defined set of arithmetic operations and is highly error-resilient. The core operations of HDC manipulate HD vectors in bulk bit-wise fashion, offering many opportunities to leverage parallelism. Unfortunately, on conventional Von-Neuman architectures, the continuous movement of HD vectors among the processor and the memory can make the cognition task prohibitively slow and energy-intensive. Hardware accelerators only marginally improve related metrics. On the contrary, only partial implementation of an HDC framework inside memory, using emerging memristive devices, has reported considerable performance/energy gains. This paper presents an architecture based on racetrack memory (RTM) to conduct and accelerate the entire HDC framework within the memory. The proposed solution requires minimal additional CMOS circuitry and uses a read operation across multiple domains in RTMs called transverse read (TR) to realize exclusive-or (XOR) and addition operations. To minimize the overhead the CMOS circuitry, we propose an RTM nanowires-based counting mechanism that leverages the TR operation and the standard RTM operations. Using language recognition as the use case demonstrates 7.8x and 5.3x reduction in the overall runtime and energy consumption compared to the FPGA design, respectively. Compared to the state-of-the-art in-memory implementation, the proposed HDC system reduces the energy consumption by 8.6x.

==> comments.tex <==
\usepackage{ifthen}
\usepackage{amssymb}
\usepackage{xcolor}

\newboolean{showcomments}
\setboolean{showcomments}{true}

% use \setboolean{showcomments}{false} anywhere in your document after
% importing this to disable the comments

\makeatletter
\newcommand{\mynote}[3]{%
  \ifthenelse{\boolean{showcomments}}{%
   \fbox{\bfseries\sffamily\scriptsize#1}%
   {\small$\blacktriangleright$\textsf{\emph{\color{#3}{#2}}}$\blacktriangleleft$}}%
  {%
   % these two lines ensure that there is no blank space inserted
   \@bsphack
   \@esphack
  }%
}
\makeatother

% One command per author:
\definecolor{asparagus}{rgb}{0.53, 0.66, 0.42}
\newcommand{\jc}[1]{\mynote{Jeronimo}{#1}{asparagus}}
\newcommand{\gh}[1]{\mynote{GH}{#1}{red}}
\newcommand{\ak}[1]{\mynote{AK}{#1}{blue}}
\newcommand{\akj}[1]{\mynote{AKJ}{#1}{violet}}
\newcommand{\so}[1]{\mynote{SO}{#1}{green}}
\newcommand{\sjl}[1]{\mynote{SJL}{#1}{orange}}



==> contents/system_overview.tex <==
\section{Overall system design}
\label{sec:overview}
% \so{introduction to this section, also what new do we introduce in this section?}\ak{This section is supposed to provide an overview of the overall system and the next section then provides detail on each component of the system.}
This section presents a high-level overview of the proposed in-RTM HDC design. Figure~\ref{fig:overview} shows the compute and memory units of the RTM, the mapping of the hypervectors, and the integration of different components. Similar to~\cite{rahimi_ISLPED_16, rahimi_TCS_17}, we use the BSC framework that has four primary operations, \textit{i.e.}, XOR and rotation for binding, majority for bundling, and XOR for the similarity check. 
% \ak{Rahimi basically uses MAP, but the implementation is the same as BSC.} 

\begin{figure}[tbh]
\centering
\includegraphics[scale=1.2]{figures/architecture.pdf}
\caption{A high-level overview of the proposed in-RTM HDC system}
\label{fig:overview}
\end{figure}

As explained in Section~\ref{subsec:hdc_bg}, each input symbol in an HDC framework is mapped to a d-dimensional base hypervector and is stored in the item memory (IM). The size of the item memory depends on the number of symbols in the classification problem. In our use case, the item memory stores $27$ hypervectors and entirely fits in DBC$_0$ of each data processing unit (DPU). The DPU stores the $d=8192$ dimensional hypervectors in a bit- and tile-interleaved fashion, as shown in Figure~\ref{fig:overview}. The most significant $512$ bits of each hypervector are stored DBC$_0$ of the cim-tile $T_0$  (which is tile$_{15}$ of subarray$_0$, cf. Figure~\ref{fig:RTM_array}) and the least significant 512 are stored in DBC$_0$ of cim-tile $T_{15}$ (tile$_{15}$ of subarray$_{15}$) respectively, in each bank of the RTM. 
% \ak{TODO: cross-check with Sebastien the sizes of all these abstractions.}

In both the training and the inference phases of the HDC, encoding is the first step. The encoding operation itself consists of 3 operations \textit{i.e.}, binding, rotation and the bundling (cf. Section~\ref{subsec:hdc_bg}). The CPU %\ak{controller, if ASIC, CPU otherwise.} 
issues instructions to sequentially input the stream of letters and fetch their corresponding base hypervectors from DBC$_0$ to the encoder module. This copying of letter hypervectors within RTM is needed because the letter hypervectors need to be preserved for later references. For instance, they can be used to recover the original/noise-free hypervectors after certain arithmetic operations that produce noisy/approximate results. The item memory --- also known as the \emph{clean-up memory} --- in such scenario is probed with the noisy hypervector, and based on the nearest neighbor's search, it outputs the original hypervector~\cite{kanerva_2009}. 

% The binding logic in the encoder module generates a new hypervector for each \emph{n-gram} (tetragram in our case), a block of $n$ consecutive letters in the input stream, and sends it to the bundler. The n-gram hypervector is produced by component-wise XORing the (permuted versions of the) letter hypervectors (cf. Section~\ref{sss:binding}) and is also d-dimensional. Consider a random tetragram \verb frog, the component-wise operation is performed on the thrice permuted hypervector $\vec{f}^3$, twice permuted hypervector $\vec{r}^2$, once permute hypervector $\vec{o}^1$ and unpermuted $\vec{g}$. %Note that S$_\text{v}$ represents the hypervector of the letter \verb S. 
% Unless otherwise mentioned, the permutation in this paper strictly refers to only one particular permutation, \textit{i.e.}, the right circular rotation by one \so{"right circular rotation" is it something classically called like this}\ak{yes, I think it is a known operation on arrays!}. 
% In the bundling operation, all n-gram hypervectors are summed together to compute a single text hypervector based on the majority operation.%\so{why are we saying multiplying/XORing and summed when we only do the majority}\ak{No, they are different operations. We do XOR for mul and majority for the sum and thresholding part.}

In the training phase of the HDC, the computed text hypervector is associated with its corresponding language and is stored in the associative memory location of the RTM (cf. Figure~\ref{fig:overview})\ak{this part is still missing in the figure!}. In the inference phase, the text hypervector referred to as the \emph{query hypervector} is forwarded to the similarity search module to compute and compare its similarity score with all language hypervectors. The similarity search module computes the Hamming distance of the query hypervector with each language hypervector by performing the XOR and population count operations, respectively. While the operations within the encoding module are pipelined, the encoding and the similarity search modules can not be pipelined for a single instance of the inference because the similarity search is only performed when the encoding operation for the entire text is completed. 

% to count the dissimilar components/dimensions in Q$_\text{v}$ and each hypervector in the associative memory. For our case study, we have 21 language vectors corresponding to the 21 languages. Let $\Gamma$ be the set representing all language vectors in the associative memory, then the Hamming distance hamm\_d( Q$_\text{v}$, $l_\text{v}$ ) $\forall l_\text{vi} \text{ } \in \Gamma$ is computed and the language vector with the minimum hamm\_d is forwarded as the output.


==> response_bib.tex <==
\begin{thebibliography}{9}

\bibitem{pieee}
R. Bläsing et al., "Magnetic Racetrack Memory: From Physics to the Cusp of Applications Within a Decade," in \textit{Proceedings of the IEEE}, vol. 108, no. 8, pp. 1303-1321, Aug. 2020, doi: 10.1109/JPROC.2020.2975719.

\bibitem{dracc}
Q. Deng et al., "Dracc: a dram based accelerator for accurate cnn inference"
\textit{Proceedings of the 55th Annual Design Automation Conference}, 2018


\bibitem{HDNA}
M. Imani, T. Nassar, A. Rahimi and T. Rosing, "HDNA: Energy-efficient DNA sequencing using hyperdimensional computing," \textit{IEEE EMBS International Conference on Biomedical \& Health Informatics (BHI)}, 2018, pp. 271-274, doi: 10.1109/BHI.2018.8333421.

\bibitem{thrifty}
S. Gupta et al., "THRIFTY: Training with Hyperdimensional Computing across Flash Hierarchy," \textit{IEEE/ACM International Conference On Computer Aided Design (ICCAD)}, 2020, pp. 1-9.

\bibitem{voiceHD}
M. Imani, D. Kong, A. Rahimi and T. Rosing, "VoiceHD: Hyperdimensional Computing for Efficient Speech Recognition," \textit{IEEE International Conference on Rebooting Computing (ICRC)}, 2017, pp. 1-8, doi: 10.1109/ICRC.2017.8123650.

\bibitem{hdc-review}
Ge, L., \& Parhi, K. K. (2020). "Classification using hyperdimensional computing: A review.", \textit{IEEE Circuits and Systems Magazine}, 20(2), 30-47.

\bibitem{hdc-comp}
Hassan, E., Halawani, Y., Mohammad, B., \& Saleh, H. "Hyper-Dimensional Computing Challenges and Opportunities for AI Applications.", textit{IEEE Access}, 2021

\bibitem{kanerva}
Kanerva, P. (2009). "Hyperdimensional computing: An introduction to computing in distributed representation with high-dimensional random vectors.", \textit{Cognitive computation}, 1(2), 139-159.

\bibitem{rahimi_TCS}
Rahimi, A., Datta, S., Kleyko, D., Frady, E. P., Olshausen, B., Kanerva, P., \& Rabaey, J. M. (2017). "High-dimensional computing as a nanoscalable paradigm", \textit{IEEE Transactions on Circuits and Systems I: Regular Papers}, 64(9), 2508-2521.

\bibitem{VSAs}
Schlegel, K., Neubert, P., \& Protzel, P. (2020). "A comparison of vector symbolic architectures.", arXiv preprint arXiv:2001.11797.

\bibitem{training_data}
Quasthoff, U., Richter, M., \& Biemann, C. (2006, May). "Corpus Portal for Search in Monolingual Corpora", \textit{In LREC} (pp. 1799-1802).

\bibitem{HDC_FPGA}
Salamat, Sahand, Mohsen Imani, and Tajana Rosing. "Accelerating hyperdimensional computing on fpgas by exploiting computational reuse.", \textit{IEEE Transactions on Computers} 69.8 (2020): 1159-1171.

\bibitem{TRNano}
Roxy, K., Ollivier, S., Hoque, A., Longofono, S., Jones, A. K., \& Bhanja, S. (2020)."A Novel Transverse Read Technique for Domain-Wall Racetrack Memories.", \textit{IEEE Transactions on Nanotechnology}, 19, 648-652.

\bibitem{cimAdder}
Z. Wang et al., "Efficient Implementation of Boolean and Full-Adder Functions With 1T1R RRAMs for Beyond Von Neumann In-Memory Computing," in \textit{IEEE Transactions on Electron Devices}, vol. 65, no. 10, pp. 4659-4666, Oct. 2018, doi: 10.1109/TED.2018.2866048.

\bibitem{cimAdder2}
Roohi, Arman, Ramtin Zand, and Ronald F. DeMara. "A tunable majority gate-based full adder using current-induced domain wall nanomagnets." \textit{IEEE Transactions on Magnetics} 52.8 (2016): 1-7.

\bibitem{lctes}
Khan, Asif Ali, et al. "Optimizing tensor contractions for embedded devices with racetrack memory scratch-pads." \textit{Proceedings of the 20th ACM SIGPLAN/SIGBED International Conference on Languages, Compilers, and Tools for Embedded Systems}, 2019.

\bibitem{tapecache}
Venkatesan, Rangharajan, et al. "TapeCache: A high density, energy efficient cache based on domain wall memory." \textit{Proceedings of the 2012 ACM/IEEE international symposium on Low power electronics and design}, 2012.

\bibitem{ssd}
E. Park, S. Yoo, S. Lee and H. Li, "Accelerating graph computation with racetrack memory and pointer-assisted graph representation," \textit{2014 Design, Automation and Test in Europe Conference \& Exhibition (DATE)}, 2014, pp. 1-4, doi: 10.7873/DATE.2014.172.

\bibitem{gpu_registerfile}
Shuo Wang et al., "Performance-centric register file design for GPUs using racetrack memory," \textit{21st Asia and South Pacific Design Automation Conference (ASP-DAC)}, 2016, pp. 25-30, doi: 10.1109/ASPDAC.2016.7427984.

\bibitem{gpu_rf}
M. Mao, W. Wen, Y. Zhang, Y. Chen and H. Li, "Exploration of GPGPU register file architecture using domain-wall-shift-write based racetrack memory," \textit{51st ACM/EDAC/IEEE Design Automation Conference (DAC)}, 2014, pp. 1-6.

\bibitem{fusedcache}
H. Xu, Y. Alkabani, R. Melhem and A. K. Jones, "FusedCache: A Naturally Inclusive, Racetrack Memory, Dual-Level Private Cache," in \textit{IEEE Transactions on Multi-Scale Computing Systems}, vol. 2, no. 2, pp. 69-82, 1 April-June 2016, doi: 10.1109/TMSCS.2016.2536020.

\bibitem{content_addressable}
Y. Zhang, W. Zhao, J. Klein, D. Ravelsona and C. Chappert, "Ultra-High Density Content Addressable Memory Based on Current Induced Domain Wall Motion in Magnetic Track," in \textit{IEEE Transactions on Magnetics}, vol. 48, no. 11, pp. 3219-3222, Nov. 2012.

\bibitem{reconfig_mem}
Zhao, Weisheng, et al. "Racetrack memory based reconfigurable computing." \textit{2013 IEEE Faible Tension Faible Consommation}, IEEE, 2013.

\bibitem{dwspeed}
Kim, K.-J. et al. 
"Fast domain wall motion in the vicinity of the angular momentum compensation temperature of ferrimagnets", \textit{Nature Material} 16, 1187–1192 (2017).

\bibitem{ohsawa2018}
Ohsawa, Y. et al. in 2018 IEEE 2nd Electron Devices Technology and Manufacturing Conference (EDTM) 214–216 (2018).

\bibitem{stuart1.0} 
Parkin, S. S., Hayashi, M., and Thomas, L. (2008). "Magnetic domain-wall racetrack memory", \textit{Science}, 320(5873), 190-194.

\bibitem{spindevices} 
Puebla, J., Kim, J., Kondou, K., and Otani, Y. (2020). 
"Spintronic devices for energy-efficient data storage and energy harvesting",  \textit{Communications Materials}, 1(1), 1-9.

\bibitem{lee1999}
L. H. Lee, B. Moyer and J. Arends.
"Instruction fetch energy reduction using loop caches for embedded applications with small tight loops",
\textit{Proceedings of the International Symposium on Low power Electronics and Design}, 1999

\bibitem{filterCache1997}
J. Kin, M. Gupta and W. H. Mangione-Smith.
"The filter cache: an energy efficient memory structure",
\textit{Proceedings of the Annual International Symposium on Microarchitecture}, 1997

\bibitem{park2010}
J. Park, J. Balfour and W. J. Dally.
"Fine-grain dynamic instruction placement for L0 scratch-pad memory",
\textit{Proceedings of the International Conference on Compilers, Architectures and Synthesis for Embedded Systems}, 2010

\bibitem{blasing2018exchange}
R. Bl{\"a}sing, T. Ma, S.-H. Yang, C. Garg, F. K. Dejene, A. T N'Diaye, G. Chen, K. and Liu, and S. Parkin.
"Exchange coupling torque in ferrimagnetic Co/Gd bilayer maximized near angular momentum compensation temperature",
\textit{Nature communications}, 2018

\bibitem{tomasello2017}
R. Tomasello, V. Puliafito, E. Martinez, A. Manchon, M. Ricci, M. Carpentieri and G. Finocchio.
"Performance of synthetic antiferromagnetic racetrack memory: domain wall versus skyrmion",
\textit{Journal of Physics D: Applied Physics}, 2017

\bibitem{gao2021placement}
S. Gao, S. Gu, R. Xu, E H.-M. Sha and Q. Zhuge.
"Performance optimization for parallel systems with shared DWM via retiming, loop scheduling, and data placement",
\textit{Journal of Systems Architecture}, 2021

\bibitem{khouzani2019DWMcache}
H. A. Khouzani, C. Yang.
"Tuning track-based NVM caches for low-power IoT devices", \textit{Proceedings of the Great Lakes Symposium on VLSI}, 2019

\bibitem{xu2020SRAMandRTM}
R. Xu, E H.-M. Sha, Q. Zhuge, S. Gu, L. Shi.
"Optimizing data placement for hybrid SPM with SRAM and racetrack memory",
\textit{IEEE International Conference on Computer Design}, 2020


\bibitem{stuart4.0}
Parkin, Stuart and Yang, See-Hun. "Memory on the racetrack", 
\textit{Nature nanotechnology}, 2015

\bibitem{zhang2015}
C. Zhang et al., "Hi-fi playback: Tolerating position errors in shift operations of racetrack memory", \textit{ACM/IEEE International Symposium on Computer Architecture}, 2015

\bibitem{Ollivier2019}
S. Ollivier, D. Kline, R. Kawsher, R. Melhem, S. Banja and A. K. Jones, "Leveraging Transverse Reads to Correct Alignment Faults in Domain Wall Memories", \textit{49th Annual IEEE/IFIP International Conference on Dependable Systems and Networks}, 2019

\bibitem{archer2020foosball}
S. Archer, G. Mappouras, R. Calderbank and D. Sorin. "Foosball coding: correcting shift errors and bit flip errors in 3D racetrack memory", \textit{IEEE/IFIP International Conference on Dependable Systems and Networks}, 2020

\bibitem{fully_serial_RTM}
J. Wang et al., "An Automatic-Addressing Architecture with Fully Serialized Access in Racetrack Memory for Energy-Efficient CNNs", \textit{IEEE Transactions on Computers}, 2020.

\bibitem{acceleration_HDC}
S. Salamat et al.,"Accelerating hyperdimensional computing on fpgas by exploiting computational reuse"
\textit{IEEE Transactions on Computers}, 2020
\bibitem{PCM_HDC}
G. Karunaratne, et al. "In-memory hyperdimensional computing.", \textit{Nature Electronics}, (2020)

\bibitem{F5-HD}
S.Salamat et al. "F5-hd: Fast flexible fpga-based framework for refreshing hyperdimensional computing." \textit{ACM/SIGDA International Symposium on Field-Programmable Gate Arrays}, 2019

\bibitem{HDC_nanoscale}
A. Rahimi et al. "High-dimensional computing as a nanoscalable paradigm." \textit{IEEE Transactions on Circuits and Systems I}, 2017

\end{thebibliography}

==> response_bib2.tex <==
\begin{thebibliography}{9}

\bibitem{pulpVSpcm}
G. Karunaratne et al., "Energy Efficient In-Memory Hyperdimensional Encoding for Spatio-Temporal Signal Processing," in \textit{IEEE Transactions on Circuits and Systems II: Express Briefs}, vol. 68, no. 5, pp. 1725-1729, May 2021, doi: 10.1109/TCSII.2021.3068126.

\bibitem{HDNA}
M. Imani, T. Nassar, A. Rahimi and T. Rosing, "HDNA: Energy-efficient DNA sequencing using hyperdimensional computing," \textit{IEEE EMBS International Conference on Biomedical \& Health Informatics (BHI)}, 2018, pp. 271-274, doi: 10.1109/BHI.2018.8333421.

\bibitem{thrifty}
S. Gupta et al., "THRIFTY: Training with Hyperdimensional Computing across Flash Hierarchy," \textit{IEEE/ACM International Conference On Computer Aided Design (ICCAD)}, 2020, pp. 1-9.

\bibitem{HDC_FPGA}
Salamat, Sahand, Mohsen Imani, and Tajana Rosing. "Accelerating hyperdimensional computing on fpgas by exploiting computational reuse.", \textit{IEEE Transactions on Computers} 69.8 (2020): 1159-1171.

\bibitem{hpca}
M. Imani et al., "Revisiting HyperDimensional Learning for FPGA and Low-Power Architectures," 2021 IEEE International Symposium on High-Performance Computer Architecture (HPCA), 2021, pp. 221-234, doi: 10.1109/HPCA51647.2021.00028.

\bibitem{hdc_C}
Michael Hersche et al. HDlib, "https://github.com/skurella/hdlib", Accessed: 2022-02-22.

\bibitem{Hermes}
R. Khaddam-Aljameh et al., ``HERMES-Core--A 1.59-TOPS/mm$^2$ PCM on 14-nm CMOS In-Memory Compute Core Using 300-ps/LSB Linearized CCO-Based ADCs" in \textit{IEEE Journal of Solid-State Circuits}, 2022

\bibitem{PIRM}
S. Ollivier et al., ``PIRM: Processing In Racetrack Memories" in \textit{arXiv preprint arXiv:2108.01202}, 2021.

\bibitem{CNN_DWM}
B. Liu et al. ``An
efficient racetrack memory-based Processing-in-memory architecture for convolutional neural networks.'' In \textit{ISPA/IUCC}. IEEE, 2017, 383–390.

\end{thebibliography}
